Dataset Condensation with Latent Space Knowledge Factorization and Sharing

In this paper, we introduce a novel approach for systematically solving dataset condensation problem in an efficient manner by exploiting the regularity in a given dataset. Instead of condensing the dataset directly in the original input space, we assume a generative process of the dataset with a set of learnable codes defined in a compact latent space followed by a set of tiny decoders which maps them differently to the original input space. By combining different codes and decoders interchangeably, we can dramatically increase the number of synthetic examples with essentially the same parameter count, because the latent space is much lower dimensional and since we can assume as many decoders as necessary to capture different styles represented in the dataset with negligible cost. Such knowledge factorization allows efficient sharing of information between synthetic examples in a systematic way, providing far better trade-off between compression ratio and quality of the generated examples. We experimentally show that our method achieves new state-of-the-art records by significant margins on various benchmark datasets such as SVHN, CIFAR10, CIFAR100, and TinyImageNet.

==> tables/imagenet_subset.tex <==
\begin{table}[t!]
	\caption{\small \textbf{ImageNet-subset experiments.} RNAP, RN18, and ENB0 denote ResNetAP-10, ResNet-18, and EfficientNet-B0, respectively. We train on RNAP and evaluate on the three architectures.} \label{tbl:imagenet_subset}
	\vspace{-0.1in}
	\begin{center}
	    \small
        \resizebox{\linewidth}{!}{
		\begin{tabular}{c|x{0.35in}x{0.35in}x{0.35in}|x{0.35in}x{0.35in}x{0.35in}|x{0.35in}x{0.35in}x{0.35in}|x{0.35in}x{0.35in}x{0.35in}}
			\toprule
			 Dataset &  \multicolumn{6}{c|}{ImageNet-10} & \multicolumn{6}{c}{ImageNet-100} \\
			 \hline
			 Imgs / Cls &  \multicolumn{3}{c|}{1} &  \multicolumn{3}{c|}{10} & \multicolumn{3}{c|}{1} & \multicolumn{3}{c}{10} \\
			  Test Arch. & RNAP & RN18 & ENB0 & RNAP & RN18 & ENB0 & RNAP & RN18 & ENB0 & RNAP & RN18 & ENB0 \\
			\hline
			\hline
			DSA
			& xx.x\tiny$\pm$x.x$\ $
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			\\
			DM
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			\\
			IDC
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			\\
			\textbf{KFS (ours)}
			& \textbf{xx.x\tiny$\pm$x.x}
			& \textbf{xx.x\tiny$\pm$x.x}
			& \textbf{xx.x\tiny$\pm$x.x}
			& \textbf{xx.x\tiny$\pm$x.x}
			& \textbf{xx.x\tiny$\pm$x.x}
			& \textbf{xx.x\tiny$\pm$x.x}
			& \textbf{xx.x\tiny$\pm$x.x}
			& \textbf{xx.x\tiny$\pm$x.x}
			& \textbf{xx.x\tiny$\pm$x.x}
			& \textbf{xx.x\tiny$\pm$x.x}
			& \textbf{xx.x\tiny$\pm$x.x}
			& \textbf{xx.x\tiny$\pm$x.x}
			\\
			\hline
			Full dataset
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			& xx.x\tiny$\pm$x.x
			\\
			\bottomrule
		\end{tabular}
		}
	\end{center}
	\small
\end{table}
